On the Numerical Treatment of Interlaced Target Values -- Modeling, Optimization and Simulation of Regulating Valves in Gas Networks

Due to the current and foreseeable shifts in energy production, the trading and transport operations of gas will become more dynamic, volatile, and hence also less predictable. Therefore, computer-aided support in terms of rapid simulation and control optimization will further broaden its importance for gas network dispatching. In this paper, we aim to contribute and openly publish two new mathematical models for regulators, also referred to as control valves, which together with compressors make up the most complex and involved types of active elements in gas network infrastructures. They provide full direct control over gas networks but are in turn controlled via target values, also known as set-point values, themselves. Our models incorporate up to six dynamical target values to define desired transient states for the elements' local vicinity within the network. That is, each pair of every two target values defines a bounding box for the inlet pressure, outlet pressure as well as the passing mass flow of gas. In the proposed models, those target values are prioritized differently and are constantly in competition with each other, which can only be resolved dynamically at run-time of either a simulation or optimization process. Besides careful derivation, we compare simulation and optimization results with predictions of the commercial simulation tool SIMONE.

==> commands.tex <==
\RequirePackage{xspace}
\RequirePackage{accents}

%%-------------------------------------------------------------
%% Abbreviations
%%-------------------------------------------------------------
\newcommand{\myie}{i.e.}
\newcommand{\myIe}{I.e.}
\newcommand{\myeg}{e.g.}
\newcommand{\myst}{s.t.\ }
\newcommand{\myWlog}{W.l.o.g.\ }
\newcommand{\mywlog}{w.l.o.g.\ }
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% nice underbar, needs 'accents' package
%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\ubar}[1]{\underaccent{\bar}{{#1}}}

\newcommand{\ub}[1]{\ensuremath{\bar{#1}}\xspace}
\newcommand{\lb}[1]{\ensuremath{\ubar{#1}}\xspace}
\newcommand{\powerset}{\ensuremath{\mathcal{P}}\xspace}

%%----------------------------------------------------------
%% all used mathcal letters
%%----------------------------------------------------------
% A - arcs
% C - compressor configurations
% F - flow directions
% G - fence groups
% H - configuration facets(hyperplanes)
% M - machines (maybe unify with U?)
% O - operation modes
% P - power set
% Q - valid operation mode/flowdirection combinations
% S - Simple states
% T - time steps
% U - units (maybe unify with M?)
% V - vertices
% W - flow direction conditions

%%-----------------------------------------------------------
%% Graph
%%----------------------------------------------------------
\newcommand{\graph}{\ensuremath{G}\xspace}
\newcommand{\generalGraph}{\ensuremath{\graph=(\setVertices,\setArcs)}\xspace}
\newcommand{\netmodelGraph}{\ensuremath{\graph=(\setVertices,\setPipes \cup \setRegulators \cup \setValves \cup \setArtificialLinks)}\xspace}

% nodes
\newcommand{\setVertices}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\setVerticesAll}{\ensuremath{\setVertices = \setBoundaryNodes \cup \setInnerNodes}\xspace}
\newcommand{\setEntries}{\ensuremath{\setVertices^{+}}\xspace}
\newcommand{\setExits}{\ensuremath{\setVertices^{-}}\xspace}
\newcommand{\setBoundaryNodes}{\ensuremath{\setVertices^\mathrm{b}}\xspace}
\newcommand{\setBoundaryNodesAll}{\ensuremath{\setEntries \cup \setExits}\xspace}
\newcommand{\setInnerNodes}{\ensuremath{\setVertices^{0}}\xspace}
\newcommand{\setFenceNodes}{\ensuremath{\setVertices^{\mathrm{fn}}}\xspace}
\newcommand{\setFenceNodesNaviStation}[1]{\ensuremath{\setFenceNodes_{i}}\xspace}
\newcommand{\setArtificialNodes}{\ensuremath{\setVertices^{\mathrm{ar}}}\xspace}
\newcommand{\setArtificialNodesNaviStation}[1]{\ensuremath{\setArtificialNodes_{#1}}\xspace}

% arcs
\newcommand{\setArcs}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\setArcsAllStationModel}{\ensuremath{\setArcs = \setPipes \cup \setValves \cup \setResistors \cup \setRegulators \cup \setCompressorStations}\xspace}
\newcommand{\setPipes}{\ensuremath{\setArcs^{\mathrm{pi}}}\xspace}
\newcommand{\setRegulators}{\ensuremath{\setArcs^{\mathrm{rg}}}\xspace}
\newcommand{\setValves}{\ensuremath{\setArcs^{\mathrm{va}}}\xspace}
\newcommand{\setValvesNS}{\ensuremath{\setArcs^{\mathrm{va-s}}}\xspace}
\newcommand{\setResistors}{\ensuremath{\setArcs^{\mathrm{rs}}}\xspace}
\newcommand{\setCompressorStations}{\ensuremath{\setArcs^{\mathrm{cs}}}\xspace}

% station model specific arcs
\newcommand{\setRegulatorsControllable}{\ensuremath{\setArcs^{\mathrm{rg-c}}}\xspace}
\newcommand{\setRegulatorsNonControllable}{\ensuremath{\setArcs^{\mathrm{rg-nc}}}\xspace}
\newcommand{\setRegulatorsNonControllableActive}{\ensuremath{\setArcs^{\mathrm{rg-nca}}}\xspace}
\newcommand{\setRegulatorsNonControllableFixed}{\ensuremath{\setArcs^{\mathrm{rg-ncf}}}\xspace}
\newcommand{\setRegulatorsNonControllableAll}{\ensuremath{\setRegulatorsNonControllable := \setRegulatorsNonControllableActive\cup\setRegulatorsNonControllableFixed}\xspace}

% special compressor station sets
\newcommand{\setCompressorUnits}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\setCompressorUnitsI}[1]{\ensuremath{\setCompressorUnits_{#1}}\xspace}
\newcommand{\setCompressorConfigurations}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setCompressorConfigurationsUsingUnit}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setConfigurationFacets}[1]{\ensuremath{\mathcal{H}_{#1}}\xspace}

% navi station specific (net model)
\newcommand{\naviStationGraph}[1]{\ensuremath{G}_{#1}\xspace}
\newcommand{\naviStationGraphAll}[1]{\ensuremath{\naviStationGraph{#1}=(\setVerticesNaviStation{#1},\setArtificialLinksNaviStation{#1})\xspace}}
\newcommand{\setVerticesNaviStation}[1]{\ensuremath{\setVertices}_{#1}\xspace}
\newcommand{\setArtificialLinksNaviStation}[1]{\ensuremath{\setArcs^{\mathrm{ar}}}_{#1}\xspace}
\newcommand{\nNaviStations}{\ensuremath{m}\xspace}

% navi station specific (station model)
\newcommand{\setNSModes}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\setNSValidPairs}{\ensuremath{\mathcal{Q}}\xspace} % valid pairs of operation modes and flow directions
\newcommand{\setNSFenceGroups}{\ensuremath{\mathcal{G}}\xspace}
% old commands, deprecated, just used to create the latexdiff for the stationModelPaper
\newcommand{\setOldNSValidPairs}{\ensuremath{\mathcal{OF}}\xspace}
\newcommand{\setOldNSFenceGroups}{\ensuremath{\mathcal{FG}}\xspace}
% end of old commands
\newcommand{\setBoundaryNodesExitP}{\ensuremath{\setVertices^\mathrm{b-ex}}\xspace}

%%-----------------------------------------------------------
%% Time
%%----------------------------------------------------------
\newcommand{\setTimesteps}{\ensuremath{\mathcal{T}_0}\xspace}
\newcommand{\setTimestepsNoZero}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\nTimesteps}{\ensuremath{k}\xspace}
\newcommand{\setTimestepsAll}{\ensuremath{\setTimesteps := \{0, \dots, \nTimesteps\}}\xspace}
\newcommand{\setTimestepsNoZeroAll}{\ensuremath{\setTimestepsNoZero := \setTimesteps\setminus\{0\}}\xspace}
\newcommand{\granularity}{\ensuremath{\tau}\xspace}
\newcommand{\granularityI}[1]{\ensuremath{\granularity(#1)}\xspace}

%%-----------------------------------------------------------
%% Supplies and demands
%%----------------------------------------------------------
\newcommand{\inflow}{\ensuremath{d}}
\newcommand{\paramInflowValue}[2]{\ensuremath{D_{#1,#2}}\xspace}
\newcommand{\paramSupplyValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramDemandValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramSupplyUB}[2]{\ensuremath{\ub{D}_{#1,#2}}\xspace}
\newcommand{\paramDemandUB}[2]{\ensuremath{\lb{D}_{#1,#2}}\xspace}
\newcommand{\inflowI}[1]{\ensuremath{\inflow_{#1}}\xspace}
\newcommand{\paramInflowValueUB}[2]{\ensuremath{\ub{\inflow}_{#1,#2}}\xspace}
\newcommand{\paramInflowValueLB}[2]{\ensuremath{\lb{\inflow}_{#1,#2}}\xspace}
\newcommand{\varSupplyValue}[2]{\ensuremath{\varInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \varInflowValue
\newcommand{\varDemandValue}[2]{\ensuremath{\varInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \varInflowValue

% station model demands for inflow and pressure
\newcommand{\demandPressure}[1]{\ensuremath{\hat{\press}_{#1}}\xspace}
\newcommand{\demandInflow}[1]{\ensuremath{\hat{\inflow}_{#1}}\xspace}

%%-----------------------------------------------------------
%% Pressure
%%----------------------------------------------------------
\newcommand{\press}{\ensuremath{p}\xspace}
\newcommand{\pressI}[1]{\ensuremath{\press_{#1}}\xspace}
\newcommand{\pressUB}[1]{\ensuremath{\ub{\press}_{#1}}\xspace}
\newcommand{\pressLB}[1]{\ensuremath{\lb{\press}_{#1}}\xspace}
\newcommand{\inflowPressUB}[1]{\ensuremath{\paramPressUB{#1}^{\mathrm{act}}}\xspace} % act => active
\newcommand{\inflowPressLB}[1]{\ensuremath{\paramPressLB{#1}^{\mathrm{act}}}\xspace} % act => active

%%-----------------------------------------------------------
%% Flow
%%----------------------------------------------------------
\newcommand{\mFlow}{\ensuremath{q}\xspace}
\newcommand{\mFlowI}[1]{\ensuremath{\mFlow_{#1}}\xspace}
\newcommand{\mFlowFwd}[1]{\ensuremath{\mFlow{#1}^{\rightarrow}}\xspace}
\newcommand{\mFlowBwd}[1]{\ensuremath{\mFlow{#1}^{\leftarrow}}\xspace}
\newcommand{\mFlowUB}[1]{\ensuremath{\ub{\mFlow}_{#1}}\xspace}
\newcommand{\mFlowLB}[1]{\ensuremath{\lb{\mFlow}_{#1}}\xspace}
\newcommand{\fenceFlow}[1]{\ensuremath{\varArcFlow{#1}^\mathrm{fn}}\xspace}

%%-----------------------------------------------------------
%% Netmodel Navi Station
%%----------------------------------------------------------
\newcommand{\setArtificialLinks}{\ensuremath{\setArcs^{\mathrm{ar}}}\xspace}
\newcommand{\setShortcuts}{\ensuremath{\setArcs^{\mathrm{ar-sc-bi}}}\xspace}
\newcommand{\setShortcutsNaviStation}[1]{\ensuremath{\setShortcuts_{#1}}\xspace}
\newcommand{\setRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{ar-rg}}}\xspace}
\newcommand{\setRegulatorArcsNaviStation}[1]{\ensuremath{\setRegulatorArcs_{#1}}\xspace}
\newcommand{\setCompressorArcs}{\ensuremath{\setArcs^{\mathrm{ar-cp}}}\xspace}
\newcommand{\setCompressorArcsNaviStation}[1]{\ensuremath{\setCompressorArcs_{#1}}\xspace}
\newcommand{\setCombinedArcs}{\ensuremath{\setArcs^{\mathrm{ar-cb}}}\xspace}
\newcommand{\setCombinedArcsNaviStation}[1]{\ensuremath{\setCombinedArcs_{#1}}\xspace}

\newcommand{\setBiRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{ar-rg-bi}}}\xspace}
\newcommand{\setBiRegulatorArcsNaviStation}[1]{\ensuremath{\setBiRegulatorArcs_{#1}}\xspace}
\newcommand{\setBiCompressorArcs}{\ensuremath{\setArcs^{\mathrm{ar-cp-bi}}}\xspace}
\newcommand{\setBiCompressorArcsNaviStation}[1]{\ensuremath{\setBiCompressorArcs_{#1}}\xspace}
\newcommand{\setBiCombinedArcs}{\ensuremath{\setArcs^{\mathrm{ar-cb-bi}}}\xspace}
\newcommand{\setBiCombinedArcsNaviStation}[1]{\ensuremath{\setBiCombinedArcs_{#1}}\xspace}

\newcommand{\setDirectedArcs}{\ensuremath{\setArcs^{\mathrm{ar-di}}}\xspace}
\newcommand{\setDirectedArcsNaviStation}[1]{\ensuremath{\setDirectedArcs_{#1}}\xspace}
\newcommand{\setBiArcs}{\ensuremath{\setArcs^{\mathrm{ar-bi}}}\xspace}
\newcommand{\setBiArcsNaviStation}[1]{\ensuremath{\setBiArcs_{#1}}\xspace}
\newcommand{\setCompressingArcs}{\ensuremath{\setArcs^{\mathrm{ar-co}}}\xspace}
\newcommand{\setCompressingArcsNaviStation}[1]{\ensuremath{\setCompressingArcs_{#1}}\xspace}

\newcommand{\setSimpleStates}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\setSimpleStatesNaviStation}[1]{\ensuremath{\mathcal{S}_{#1}}\xspace}
\newcommand{\simpleState}{\ensuremath{s}\xspace}
\newcommand{\simpleStateFlowDirections}{\ensuremath{\simpleState^{\flowDirection}}\xspace}
\newcommand{\simpleStateLinksMandatoryActive}{\ensuremath{\simpleState^{on}}\xspace}
\newcommand{\simpleStateLinksMandatoryInactive}{\ensuremath{\simpleState^{off}}\xspace}

\newcommand{\varActivation}[2]{\ensuremath{x_{#1,#2}}\xspace}
\newcommand{\varFlowDirectionActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varSimpleStateActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkActivationFwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\rightarrow}}\xspace}
\newcommand{\varArtificialLinkActivationBwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\leftarrow}}\xspace}
\newcommand{\varCombinedLinkRegulatingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{rg}}}\xspace}
\newcommand{\varCombinedLinkCompressingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{cp}}}\xspace}

\newcommand{\varChange}[2]{\ensuremath{\delta_{#1,#2}}\xspace}
\newcommand{\varFlowDirectionChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varSimpleStateChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkChangeOn}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{on}}}\xspace}
\newcommand{\varArtificialLinkChangeOff}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{off}}}\xspace}

\newcommand{\setFlowDirectionConditions}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\setFlowDirectionConditionsNaviStation}[1]{\ensuremath{\setFlowDirectionConditions_{i}}\xspace}

%%-----------------------------------------------------------
%% Machines, Power, Compression Ratio, and Betriebsvolumenstrom
%%-----------------------------------------------------------
\newcommand{\setMachinesNaviStation}[1]{\ensuremath{\mathcal{M}}_{#1}\xspace}
\newcommand{\setMachinesNaviStationOnLink}[2]{\ensuremath{\setMachinesNaviStation{#1}^{#2}}\xspace}
\newcommand{\generalMachine}{\ensuremath{m}\xspace}
\newcommand{\machine}[1]{\ensuremath{\generalMachine_{#1}}\xspace}

\newcommand{\varAssignMachineToLink}[3]{\ensuremath{y_{#1,#2,#3}}\xspace}

\newcommand{\paramMaxNumberMachinesLink}{\ensuremath{M_a^{\mathrm{max}}}\xspace}
\newcommand{\paramMaxCompressionRatio}[2]{\ensuremath{R_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxPower}[2]{\ensuremath{\power_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxBetriebsVolumenstrom}[2]{\ensuremath{\volumetricFlow_{\machine{#1},#2}}\xspace}

\newcommand{\varCompressionRatio}[2]{\ensuremath{r_{#1,#2}}\xspace}
\newcommand{\varPower}[2]{\ensuremath{\pi_{#1,#2}}\xspace}
\newcommand{\varBetriebsVolumenstrom}[2]{\ensuremath{\omega_{#1,#2}}\xspace}
\newcommand{\varMaxPower}[2]{\ensuremath{\varPower{#1}{#2}^{max}}\xspace}
\newcommand{\varMaxBetriebsVolumenstrom}[2]{\ensuremath{\varBetriebsVolumenstrom{#1}{#2}^{max}}\xspace}

\newcommand{\paramMaxCompressionRatioLink}[2]{\ensuremath{\ub{R}_{#1,#2}}\xspace}
\newcommand{\paramPressureUBCompression}[2]{\ensuremath{\paramPressureUB{#1}{#2}^{\mathrm{out}}}\xspace}


%%-----------------------------------------------------------
%% Smoothing
%%-----------------------------------------------------------

\newcommand{\generalSmoothing}{\ensuremath{\delta}\xspace}
\newcommand{\varSmoothingPressurePos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press+}}\xspace}
\newcommand{\varSmoothingPressureNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press-}}\xspace}
\newcommand{\varSmoothingInflowPos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow+}}\xspace}
\newcommand{\varSmoothingInflowNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow-}}\xspace}

%%-----------------------------------------------------------
%% Flow Direction (used in both models)
%%-----------------------------------------------------------
\newcommand{\setFlowDirectionsNavi}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\setFlowDirectionsNaviStation}[1]{\ensuremath{\setFlowDirectionsNavi_{#1}}\xspace}
\newcommand{\flowDirection}{\ensuremath{f}\xspace}
\newcommand{\flowDirectionEntries}{\ensuremath{\flowDirection^{+}}\xspace}
\newcommand{\flowDirectionExits}{\ensuremath{\flowDirection^{-}}\xspace}
\newcommand{\pressUBExitFG}[1]{\ensuremath{\ub{\press}_{#1}^{\mathrm{exit}}}\xspace}

%%-----------------------------------------------------------
%% Mode variables
%%----------------------------------------------------------
\newcommand{\mode}{\ensuremath{m}\xspace}
\newcommand{\modeOp}[1]{\ensuremath{\mode_{#1}^\mathrm{op}}\xspace}
\newcommand{\modeCl}[1]{\ensuremath{\mode_{#1}^\mathrm{cl}}\xspace}
\newcommand{\modeBy}[1]{\ensuremath{\mode_{#1}^\mathrm{by}}\xspace}
\newcommand{\modeAc}[1]{\ensuremath{\mode_{#1}^\mathrm{ac}}\xspace}
\newcommand{\modeCv}[1]{\ensuremath{\mode_{#1}^\mathrm{cvcl}}\xspace} % closed because of a flap trap
\newcommand{\modeFix}[1]{\ensuremath{\mode_{#1}^\mathrm{fix}}\xspace} % fixed mode for non-controllable regulators
\newcommand{\modeX}[1]{\ensuremath{\mode_{#1}^\mathrm{x}}\xspace}
\newcommand{\cfg}[1]{\ensuremath{\mode_{#1}^\mathrm{cf}}\xspace}
\newcommand{\opMode}[1]{\ensuremath{\mode_{#1}^\mathrm{om}}\xspace}
\newcommand{\flowDir}[1]{\ensuremath{\mode_{#1}^\mathrm{fd}}\xspace}


%%-----------------------------------------------------------
%% Mode specific pressure and flow variables
%%----------------------------------------------------------
\newcommand{\pressBy}[1]{\ensuremath{\pressI{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowBy}[1]{\ensuremath{\mFlowI{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfg}[1]{\ensuremath{\mFlowI{#1}^\mathrm{cf}}\xspace}
%% upper bounds for all of them
\newcommand{\pressByUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{cf}}\xspace}
%% lower bounds for all of them
\newcommand{\pressByLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{cf}}\xspace}

%%-----------------------------------------------------------
%% Slack variables
%%----------------------------------------------------------
\newcommand{\slack}{\ensuremath{\sigma}\xspace}
\newcommand{\slackPPos}[1]{\ensuremath{\slack_{#1}^{\press+}}\xspace}
\newcommand{\slackPNeg}[1]{\ensuremath{\slack_{#1}^{\press-}}\xspace}
\newcommand{\slackQPos}[1]{\ensuremath{\slack_{#1}^{\inflow+}}\xspace}
\newcommand{\slackQNeg}[1]{\ensuremath{\slack_{#1}^{\inflow-}}\xspace}

%%-----------------------------------------------------------
%% Target values
%%----------------------------------------------------------
%% target value types
\newcommand{\PIN}{\pressI{\mathrm{in}}\xspace}
\newcommand{\POUT}{\pressI{\mathrm{out}}\xspace}
\newcommand{\MINPIN}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MAXPIN}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MINPOUT}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MAXPOUT}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MINQ}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\MAXQ}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\SETQ}{\ensuremath{\mFlowI{\mathrm{set}}}\xspace}

%% sets
\newcommand{\setTargetValues}{\ensuremath{\Gamma}\xspace} % all TVs
\newcommand{\setTargetValuesI}[1]{\ensuremath{\setTargetValues_{#1}}\xspace} % ... of some element
\newcommand{\setStaPush}{\ensuremath{\Theta}\xspace} % all stable/pushing TV combinations
\newcommand{\setStaPushI}[1]{\ensuremath{\setStaPush_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushActive}{\ensuremath{\setStaPush^\mathrm{ac}}\xspace} % all combinations for active mode
\newcommand{\setStaPushActiveI}[1]{\ensuremath{\setStaPushActive_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushOpen}{\ensuremath{\setStaPush^\mathrm{op}}\xspace} % all combinations for open mode
\newcommand{\setStaPushOpenI}[1]{\ensuremath{\setStaPushOpen_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushClosed}{\ensuremath{\setStaPush^\mathrm{cl}}\xspace} % all combinations for closed mode
\newcommand{\setStaPushClosedI}[1]{\ensuremath{\setStaPushClosed_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushXI}[1]{\ensuremath{\setStaPush^\mathrm{x}_{#1}}\xspace} % all combination for x mode for some element

%% vars
\newcommand{\tv}{\ensuremath{\tau}\xspace}
\newcommand{\tvI}[1]{\ensuremath{\tv_{#1}}\xspace}
\newcommand{\lbTVI}[1]{\ensuremath{\lb{\tv}_{#1}}\xspace}
\newcommand{\ubTVI}[1]{\ensuremath{\ub{\tv}_{#1}}\xspace}

%\newcommand{\varMINPIN}[2]{\ensuremath{\tv^{\MINPIN}_{#1,#2}}\xspace}
%\newcommand{\varMAXPIN}[2]{\ensuremath{\tv^{\MAXPIN}_{#1,#2}}\xspace}
%\newcommand{\varMINPOUT}[2]{\ensuremath{\tv^{\MINPOUT}_{#1,#2}}\xspace}
%\newcommand{\varMAXPOUT}[2]{\ensuremath{\tv^{\MAXPOUT}_{#1,#2}}\xspace}
%\newcommand{\varMINQ}[2]{\ensuremath{\tv^{\MINQ}_{#1,#2}}\xspace}
%\newcommand{\varMAXQ}[2]{\ensuremath{\tv^{\MAXQ}_{#1,#2}}\xspace}
%
%% not complete yet ...
%\newcommand{\lbMAXPIN}[2]{\ensuremath{\lb{\tv}^{\MAXPIN}_{#1,#2}}\xspace}
%\newcommand{\ubMAXPIN}[2]{\ensuremath{\ub{\tv}^{\MAXPIN}_{#1,#2}}\xspace}
%\newcommand{\lbMINPOUT}[2]{\ensuremath{\lb{\tv}^{\MINPOUT}_{#1,#2}}\xspace}
%\newcommand{\ubMINPOUT}[2]{\ensuremath{\ub{\tv}^{\MINPOUT}_{#1,#2}}\xspace}

% target value stable pushing combination variable
\newcommand{\tvCombi}{\ensuremath{\theta}\xspace}
\newcommand{\tvCombiI}[1]{\ensuremath{\tvCombi_{#1}}\xspace}
\newcommand{\funcTvPrio}{\ensuremath{\varphi}\xspace} % target value priority function
\newcommand{\funcTvPrioI}[1]{\ensuremath{\funcTvPrio(#1)}\xspace} % .. with argument


%%-----------------------------------------------------------
%% Objective change variables
%%----------------------------------------------------------
\newcommand{\objVar}{\ensuremath{\delta}\xspace}
\newcommand{\objVarI}[1]{\ensuremath{\delta_{#1}}\xspace}
\newcommand{\opModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{om}}}\xspace}
\newcommand{\unitStart}[1]{\ensuremath{\objVarI{#1}^{\mathrm{us}}}\xspace}
\newcommand{\regModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg}}}\xspace}
\newcommand{\xPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-pl}}}\xspace}
\newcommand{\xPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-pr}}}\xspace}
\newcommand{\xQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-q}}}\xspace}
\newcommand{\rgPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-pl}}}\xspace}
\newcommand{\rgPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-pr}}}\xspace}
\newcommand{\rgQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-q}}}\xspace}
\newcommand{\csPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-pl}}}\xspace}
\newcommand{\csPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-pr}}}\xspace}
\newcommand{\csQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-q}}}\xspace}

%%-----------------------------------------------------------
%% Other physical quantities
%%----------------------------------------------------------
\newcommand{\velo}{\ensuremath{v}\xspace}
\newcommand{\absVelo}[1]{\ensuremath{|\velo_{#1}|}\xspace}
\newcommand{\gasConst}{\ensuremath{R}\xspace}
\newcommand{\sGasConst}{\ensuremath{\gasConst_{\mathrm{s}}}\xspace}
\renewcommand{\temp}{\ensuremath{T}\xspace} % special adjustment for tv paper, \temp is already defined by the 'glossaries' package
\newcommand{\tempI}[1]{\ensuremath{\temp{#1}}\xspace}
\newcommand{\zFact}{\ensuremath{z}\xspace}
\newcommand{\zFactI}[1]{\ensuremath{\zFact_{#1}}\xspace}
\newcommand{\pseudoP}{\ensuremath{\press^\mathrm{c}}\xspace}
\newcommand{\pseudoT}{\ensuremath{\temp^\mathrm{c}}\xspace}
\newcommand{\molMass}{\ensuremath{M}\xspace}
\newcommand{\len}{\ensuremath{L}\xspace}
\newcommand{\lenI}[1]{\ensuremath{\len_{#1}}\xspace}
\newcommand{\area}{\ensuremath{A}\xspace}
\newcommand{\areaI}[1]{\ensuremath{\area_{#1}}\xspace}
\newcommand{\diam}{\ensuremath{D}\xspace}
\newcommand{\diamI}[1]{\ensuremath{\diam_{#1}}\xspace}
\newcommand{\slope}{\ensuremath{s}\xspace}
\newcommand{\slopeI}[1]{\ensuremath{\slope_{#1}}\xspace}
\newcommand{\fric}{\ensuremath{\lambda}\xspace}
\newcommand{\fricI}[1]{\ensuremath{\fric_{#1}}\xspace}
\newcommand{\rough}{\ensuremath{k}\xspace}
\newcommand{\roughI}[1]{\ensuremath{\rough_{#1}}\xspace}
\newcommand{\dynVisc}{\ensuremath{\eta}\xspace}
\newcommand{\gravAcc}{\ensuremath{g}\xspace}
\newcommand{\dens}{\ensuremath{\rho}\xspace}
\newcommand{\nDens}{\ensuremath{\dens_0}\xspace} % subscript is used in the code for this and should be left free, if possible
\newcommand{\vFlow}{\ensuremath{Q}\xspace}
\newcommand{\nvFlow}{\ensuremath{Q^0}\xspace}
\newcommand{\nvFlowI}[1]{\ensuremath{Q^0_{#1}}\xspace}
\newcommand{\timeDiff}{\ensuremath{\Delta_t}\xspace} %equals \tau(t) - \tau(t-1)
\newcommand{\power}{\ensuremath{P}\xspace}
\newcommand{\adEnth}{\ensuremath{H_\mathrm{ad}}\xspace}
\newcommand{\adEff}{\ensuremath{\eta_\mathrm{ad}}\xspace} % \eta is already the dyn viscosity, but it's the same in the gas book
\newcommand{\isenExp}{\ensuremath{\kappa}\xspace}

%%-----------------------------------------------------------
%% Other element parameters
%%----------------------------------------------------------
\newcommand{\height}[1]{\ensuremath{h_{#1}}\xspace}
\newcommand{\drag}[1]{\ensuremath{\zeta_{#1}}\xspace}
\newcommand{\machinePDiffUB}{\ensuremath{\ub{\Delta}_\press}\xspace}

%%-----------------------------------------------------------
%% Objective cost parameters
%%-----------------------------------------------------------
\newcommand{\cost}{\ensuremath{w}\xspace}
\newcommand{\costSlackP}{\ensuremath{\cost^{\slack\mathrm{-p}}}\xspace}
\newcommand{\costSlackQ}{\ensuremath{\cost^{\slack\mathrm{-d}}}\xspace}
\newcommand{\costOpModes}{\ensuremath{\cost^\mathrm{om}}\xspace}
\newcommand{\costUnitStarts}{\ensuremath{\cost^\mathrm{us}}\xspace}
\newcommand{\costRgModeChg}{\ensuremath{\cost^\mathrm{rg}}\xspace}
\newcommand{\costXPLChg}{\ensuremath{\cost^\mathrm{X-pl}}\xspace}
\newcommand{\costXPRChg}{\ensuremath{\cost^\mathrm{X-pr}}\xspace}
\newcommand{\costXQChg}{\ensuremath{\cost^\mathrm{X-q}}\xspace}
\newcommand{\costRgPLChg}{\ensuremath{\cost^\mathrm{rg-pl}}\xspace}
\newcommand{\costRgPRChg}{\ensuremath{\cost^\mathrm{rg-pr}}\xspace}
\newcommand{\costRgQChg}{\ensuremath{\cost^\mathrm{rg-q}}\xspace}
\newcommand{\costCsPLChg}{\ensuremath{\cost^\mathrm{cs-pl}}\xspace}
\newcommand{\costCsPRChg}{\ensuremath{\cost^\mathrm{cs-pr}}\xspace}
\newcommand{\costCsQChg}{\ensuremath{\cost^\mathrm{cs-q}}\xspace}
\newcommand{\costFlowDirectionChange}{\ensuremath{\cost^f}\xspace}
\newcommand{\costFlowDirectionChangeNaviStation}[1]{\ensuremath{\costFlowDirectionChange_{#1}}\xspace}
\newcommand{\costOriginalSimpleStateChange}{\ensuremath{\tilde{\cost}^s}\xspace}
\newcommand{\costSimpleStateChange}{\ensuremath{\cost^s}\xspace}
\newcommand{\costArtificialLinkChange}{\ensuremath{\cost^a}\xspace}
\newcommand{\costCompressingLinkOn}[1]{\ensuremath{\cost_{#1}^{\mathrm{cp-act}}}\xspace}
\newcommand{\costCompressingLinkValue}[1]{\ensuremath{\cost_{#1}^{\mathrm{cp-val}}}\xspace}
\newcommand{\costSmoothingPressure}{\ensuremath{\cost^{\mathrm{sm-p}}}\xspace}
\newcommand{\costSmoothingFlow}{\ensuremath{\cost^{\mathrm{sm-q}}}\xspace}

%%-----------------------------------------------------------
%% Number sets
%%----------------------------------------------------------
\newcommand{\setReals}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\setRealsNonNeg}{\ensuremath{\setReals_{\geq 0}}\xspace}
\newcommand{\setRealsNonPos}{\ensuremath{\setReals_{\leq 0}}\xspace}
\newcommand{\setRealsNeg}{\ensuremath{\setReals_{< 0}}\xspace}
\newcommand{\setRealsPos}{\ensuremath{\setReals_{> 0}}\xspace}
\newcommand{\setNaturalNumbers}{\ensuremath{\mathbb{N}}\xspace}
